Statistical inference under response-adaptive experimental designs: a systematic review

Response-adaptive designs, including bandit-based approaches, update treatment allocation using accrued outcomes. In this paper, we systematically reviewed how studies in health and biostatistics conducted and evaluated inference under these designs. We searched six databases for studies published from January 2010 through October 2025. Of 774 records identified, 36 studies met the inclusion criteria. We summarized them using study-level counts and structured narrative comparisons, with reporting guided by PRISMA 2020. Most studies focused on methods or designs. Evidence supporting inference came mainly from theory and simulation. Among studies for which each metric was relevant, 26 of 32 numerically evaluated power, 23 of 32 type I error, eight of 35 estimator bias, and five of 12 interval coverage. These findings suggest that studies more often quantified power and type I error than estimator bias or interval coverage. Evaluations of adaptive allocation should also examine estimation and interval performance when these are relevant to the study objective.

==> study_evidence-labels.tex <==
% Generated from study_evidence.aux by scripts/build_documents.py.
% Label numbers/pages only: no external PDF hyperlinks or bibliography state.
\makeatletter
\@namedef{r@app:full-extraction}{{E1}{1}{}{}{}}
\@namedef{r@tab:appq1}{{E1}{2}{}{}{}}
\@namedef{r@tab:appq1a2}{{E1}{2}{}{}{}}
\@namedef{r@tab:appq1b}{{E2}{5}{}{}{}}
\@namedef{r@tab:appq1b2}{{E2}{5}{}{}{}}
\@namedef{r@tab:appq2}{{E3}{12}{}{}{}}
\@namedef{r@tab:appq2a2}{{E3}{12}{}{}{}}
\@namedef{r@tab:appq2b}{{E4}{16}{}{}{}}
\@namedef{r@tab:appq3}{{E5}{19}{}{}{}}
\@namedef{r@tab:appq3a2}{{E5}{19}{}{}{}}
\@namedef{r@tab:appq3b}{{E6}{24}{}{}{}}
\@namedef{r@tab:appq4}{{E7}{26}{}{}{}}
\@namedef{r@tab:appq4a2}{{E7}{26}{}{}{}}
\@namedef{r@tab:appq4b}{{E8}{33}{}{}{}}
\@namedef{r@tab:appq4b2}{{E8}{33}{}{}{}}
\makeatother


==> supplementary_methods-labels.tex <==
% Generated from supplementary_methods.aux by scripts/build_documents.py.
% Label numbers/pages only: no external PDF hyperlinks or bibliography state.
\makeatletter
\@namedef{r@app:count-memberships}{{S2}{2}{}{}{}}
\@namedef{r@app:exclusions}{{S3}{15}{}{}{}}
\@namedef{r@app:prisma-abstract-checklist}{{S6}{24}{}{}{}}
\@namedef{r@app:prisma-checklist}{{S5}{19}{}{}{}}
\@namedef{r@app:search}{{S4}{18}{}{}{}}
\@namedef{r@app:topicmodel}{{S1}{1}{}{}{}}
\@namedef{r@tab:appexcl}{{S5}{15}{}{}{}}
\@namedef{r@tab:papersq1}{{S1}{2}{}{}{}}
\@namedef{r@tab:papersq2}{{S2}{6}{}{}{}}
\@namedef{r@tab:papersq3}{{S3}{8}{}{}{}}
\@namedef{r@tab:papersq4}{{S4}{11}{}{}{}}
\@namedef{r@tab:prismaabstractchecklist}{{S7}{24}{}{}{}}
\@namedef{r@tab:prismachecklist}{{S6}{19}{}{}{}}
\makeatother

